What is Your Favorite Gender, MLM? Gender Bias Evaluation in Multilingual Masked Language Models

Bias is a disproportionate prejudice in favor of one side against another. Due to the success of transformer-based Masked Language Models (MLMs) and their impact on many NLP tasks, a systematic evaluation of bias in these models is needed more than ever. While many studies have evaluated gender bias in English MLMs, only a few works have been conducted for the task in other languages. This paper proposes a multilingual approach to estimate gender bias in MLMs from 5 languages: Chinese, English, German, Portuguese, and Spanish. Unlike previous work, our approach does not depend on parallel corpora coupled with English to detect gender bias in other languages using multilingual lexicons. Moreover, a novel model-based method is presented to generate sentence pairs for a more robust analysis of gender bias, compared to the traditional lexicon-based method. For each language, both the lexicon-based and model-based methods are applied to create two datasets respectively, which are used to evaluate gender bias in an MLM specifically trained for that language using one existing and 3 new scoring metrics. Our results show that the previous approach is data-sensitive and not stable as it does not remove contextual dependencies irrelevant to gender. In fact, the results often flip when different scoring metrics are used on the same dataset, suggesting that gender bias should be studied on a large dataset using multiple evaluation metrics for best practice.

==> tex/Limitations.tex <==
\section{Limitations}
\label{limit}

One major limitation of our work is being limited to only five languages is one major limitation of our evaluation schema.
Generating pairs of sentences is complicated for morphologically-rich languages because changing one word leads to changing all the grammatically related words that connote gender.
Another limitation is that the gender bias evaluation has been conducted only on BERT-based models.
With advances in cross-lingual language models, examining gender bias in different languages of these cross-lingual language models might show interesting results compared to language-specific BERT-based models.
We hope to expand our methods to explore gender bias in more language models and use evaluation corpora that are not parallel.

 
